Clustering the Sketch: A Novel Approach to Embedding Table Compression

Embedding tables are used by machine learning systems to work with categorical features. In modern Recommendation Systems, these tables can be very large, necessitating the development of new methods for fitting them in memory, even during training. We suggest Clustered Compositional Embeddings (CCE) which combines clustering-based compression like quantization to codebooks with dynamic methods like The Hashing Trick and Compositional Embeddings (Shi et al., 2020). Experimentally CCE achieves the best of both worlds: The high compression rate of codebook-based quantization, but *dynamically* like hashing-based methods, so it can be used during training. Theoretically, we prove that CCE is guaranteed to converge to the optimal codebook and give a tight bound for the number of iterations required.

==> notes/cqr.tex <==
\input{../header.tex}

\author{Thomas Dybdahl Ahle, Henry Tsang}
\title{Clustered Compositional Embedding}
\begin{document}
\maketitle

Let $X \in \R^{n \times d_1}$
be some data points,
pick $T \in \R^{d_1 \times d_2}$
and let $Y = XT \in \R^{n\times d_2}$.
Assume $d_1$ is at least $d_2^2$, but possibly much more.\footnote{
We can also add some noise $Y$ to make the problem of recovering $T$ a bit more exciting, but it doesn't change much about the findings in this note.}

%In fact we assume $X$ is very sparse in $X\in \{0,1\}^{n\times d_1}$ so it can be stored in $O(n+d_1)$ memory.
%Our goal will be to efficiently retrieve $T$ from $(X,Y)$
%at least find an approximation to $\argmin_T \|XT-Y\|_2^2$ using memory that doesn't depend on $d_1$.

Obviously we can easily retrieve $T$ from $(X,Y)$ solving the least squares problem $\argmin_T \|XT-Y\|_2^2$ or otherwise.
However, assume we want to save memory, so we instead pick a random matrix
$H \in \R^{d_1\times k}$
and find
$$M_\text{cs}=\argmin_{M\in\R^{k\times d_2}} \|XHM-Y\|_2^2.$$
Then $T_{\text{cs}}=HM_\text{cs}$ is an approximation to $T$,
in so far as $H$ preserves the column space of $T$, which is likely if $k > d_2$.
Classical results from sketching shows that $H$ can be a very sparse binary matrix, so we have indeed saved memory.

While we can get useful results by picking $H$ with just one 1 per row (a so called Count Sketch matrix),
we can get much better results by computing the k-means of the rows of $T$.
Say $S_\text{km}\in\{0,1\}^{d_1\times k}$ is the assignments of the $d_1$ rows to their nearest cluster center (we don't care about the centers, only the assignment) and let $$M_\text{km}=\argmin_{M\in\R^{k\times d_2}} \|XS_\text{km}M-Y\|_2^2.$$
Then $T_\text{km}=S_\text{km}M_\text{km}$ is reliably a much better approximation to $T$ than $T_\text{cs}$, even though they use the same amount of memory.

While this is already interesting, and we would like to prove it more rigorously, what's really interesting is the following:
If we compute k-means on $T_\text{cs}$ and let $S_\text{cqr}\in\{0,1\}^{d_1\times k}$ be the assignments and $M_\text{cqr}\in\R^{k\times d_2}$ be the solution the least squares problem as before,
then $T_\text{cqr}$ is \emph{also} a better approximation to $T$ than $T_\text{cs}$ (while not quite as good as $T_\text{km}$.)
This is all in the sense that
\begin{align}
\|XT-Y\|_2 <
\|XT_\text{km}-Y\|_2 <
\|XT_\text{cqr}-Y\|_2 <
\|XT_\text{cs}-Y\|_2.
\label{eq:main}
\end{align}
In other words, it appears to be possible to improve the solution $T_\text{cs}$ found by the sketching method, by simply taking k-means and training again.

Let's analyze the memory usage, assuming $X$ and $Y$ are stored externally and retrieved in batches.
The Count-Sketch\footnote{Actually it has to be the sum of two Count-Sketch matrices. Otherwise k-means simply recovers the original $H$ and no improvement is possible. Meanwhile using a denser $H$ than two 1s per row seems unnecessary.} matrix $H$ just requires a hash function, so $O(1)$ memory.
Computing $M_\text{cs}$ can be done again in batches, taking only the memory to store $M$ which is $O(kd_2)$.
Computing k-means of $T_\text{cs}$ can be done with just oracle access to $T_\text{cs}$ (so we don't have to materialize the full $d_1\times d_2$ matrix,) taking just $O(d_1)$ memory to store the assignment and $O(kd_2)$ to store the cluster centers.
Finally computing $M_\text{cqr}$ is again $O(kd_2)$ memory.
So all together we used $O(d_1+kd_2)$ memory.
Much less than the $\Omega(d_1d_2)$ needed to compute $T$ or $T_\text{km}$.

The main question is now f we can actually prove \cref{eq:main}.
Ideally in a quantifiable version, so we know the dependence on $k$, and possibly on the distribution of $X$ and $T$.


\section{Old version}

Let $D \in \R^{d_1} \times \R^{d_2}$ be a dataset.
We are interested in $d_1 >\!> d_2$ and sometimes even
$D\in \{0,1\}^{d_1} \times \R^{d_2}$.

Traditional embedding learning is the task of finding
$T \in \R^{d_1\times d_2}$ optimizing
\begin{align}
   \argmin_{T} \sum_{(x,y)\in D} \|T^t x-y\|_2^2
   .
   \label{eq:opt}
\end{align}
This is typically done with stochastic gradient descent.
Loss functions other that $l_2$-norm are also possible, but let's focus on that for now.

However, this table $T$ may be very large.
Product or Residual Vector Quantization tries to save space by finding matrices
$M\in \R^{k \times d_2}$ and $H\in \{0,1\}^{d_1\times k}$
such that $T \approx HM$.
Or more specifically optimizing
\begin{align}
   \argmin_{H, M} \sum_{(x,y)\in D} \|HM - T\|_F^2,
   \label{eq:pq}
\end{align}
where $\|T\|_F^2 = \sum_{i,j} T_{i,j}^2$ is just the squared Frobenius norm.
In particular, if $H$ has exactly one 1 on each row, \cref{eq:pq} is just the $k$-means problem.

While this may eventually produce a cheap representation of $T$, we still need to store the entire $T$ during step 1 (\cref{eq:opt}) and step 2 (\cref{eq:pq}).
To reduce memory usage we propose the following alternative:

Let $H'\in\{-1,0,1\}^{d_1\times k'}$ be a sparse random matrix, or something else that allows cheap storage and fast vector-multiplication, like a Fast JL matrix.\footnote{
Note that we can't make $H'$ as sparse as a Count Sketch matrix, which has only one $\pm 1$ per row.
If $H'$ had only one 1 per row, the clustering/scarification step (step 2) probably wouldn't do anything useful.
}
% (Here $k'$ might equal $k$ or be a bit larger.)
Now find a matrix $M'\in\R^{k'\times d_2}$ such that $H'M'$ optimizes the same target as $T$ originally did (\cref{eq:opt}).
Then use the same k-means procedure to find $H$ and $M$ that we sought in \cref{eq:pq}.
\begin{align}
   \text{Step 1 (sketched training):}\quad
   & \argmin_{M'} \sum_{(x,y)\in D} \|(H'M')^t x-y\|_2^2
   \label{eq:step1}
   \\
   \text{Step 2 (k-means clustering):}\quad
   & \argmin_{H,M} \|H'M' - HM\|_F^2
   \label{eq:step2}
   \\
   \text{Step 3 (fine-tuning, optional):}\quad
   & \argmin_{M''} \sum_{(x,y)\in D} \|(HM'')^t x - y\|_2^2
   \label{eq:step3}
   .
\end{align}
The third step is an optional fine-tuning step in which we freeze the $H$ matrix found by k-means in step 2, and optimize the compressed table $M$ again.

Note that if we try to perform \cref{eq:step2} directly, it will fully compute $H'M'$ which takes as much memory as $T$ originally would have, and so destroys and chance of success.
We overcome this by sub-sampling which work well as long as we pick say $100k$ rows or more.
Let's ignore this issue for now though.
Also assume that we can actually store $H$ in memory, even though it has $d_1$ rows.

Now the goal is to prove that the result of \cref{eq:pq}, say $H^{(1)}M^{(1)}$ is not far from the result of \cref{eq:step2}, say $H^{(2)}M^{(2)}$.
For example we could hope that $\|H^{(1)}M^{(1)}-H^{(2)}M^{(2)}\| < \eps$ or even
\begin{align}
   \sum_{(x,y)\in D} \|(H^{(2)}M^{(2)})^t x - y\|_2^2
   \le
   \sum_{(x,y)\in D} \|(H^{(1)}M^{(1)})^t x - y\|_2^2 + \eps.
\end{align}

Actually, I write that Step 3 is optional, but maybe that's a mistake.
After all, if we don't do any fine-tuning after clustering,
why would we ever expect the results to be better than just keeping the $H'M'$ matrix? (In our case that would be the hybrid method.)
Of course one could also do fine-tuning on the PQ model, but in our experiments that seems to overfit.
So the real mystery is: Why does fine-tuning on the clustering derived from the sketched $T$ work well, but the fine-tuning from the real $T$ clustering perform badly?

\end{document}


==> sections/other_related_work.tex <==




==> sections/theory.tex <==

I kinda want to cite Erik's sparse recovery stuff?

How close are the embeddings we learn to the optimal ones?
I really don't think we can say anything about that...
We don't even know how good PQ is...
But can we say how close we get to PQ?

I think saying getting close to PQ is fine.
In fact, we can move the PQ inference graph here.
On the other hand, 
I am still disturbed by the failures of PQ seed.
Doing PQ from the full embedding table was supposed to give us the best results.
We can similarly move that part from section 6 to here.


%\begin{theorem}
The embeddings learned by CCE are 
%\end{theorem}

Can we give some simple theorem describing how good our embeddings are?
Maybe we can refer to sparse JL 

\subsection{Intuition based on subspaces}

Embedding a vector is equivalent to performing a linear transformation.
If $v$ is a one-hot, multi-hot or general sparse vector, then the embedding of $v$ into $d$ dimensions is just $Wv$, where $W$ is the embedding matrix.
(Transposed as needed.)

The fact that we are imposing a linear transformation down to $d$ dimensions, means that we only care about a $d$ dimensional linear subspace of the original space.

\paragraph{Enter subspace embeddings}
It can be shown that a random matrix with enough rows (function of $d$) will preserve any linear subspace of dimension $d$ up to a factor $1\pm \epsilon$ in the norm of the vectors in the subspace.
See~\cite{DBLP:journals/fttcs/Woodruff14}.

This means that a random matrix $S$, with not too many rows, such that any $W$ can be written as $W' S$, where $W'$ has much fewer columns than $W$.
And what's just as important, there is no matrix $W''$ that works ``better'' than $W'$, since every other subspace is also preserved.
This is important to guarantee that the optimizer doesn't suddenly find a different optimum that doesn't correspond to the original unsketched case.

In our world, this means that we first multiply $S$ on $v$, and then learn $W'$ using the same technique as before, then the network is able to find exactly the same embedding, only this time with much fewer parameters.

But isn't it expensive/memory inefficient to store $S$?
Well, it turns out that $S$ can be very sparse.

In the paper~\cite{DBLP:conf/focs/NelsonN13} Nelson, Jelani, and Huy L. Nguyên show how to do exactly that.
Even a simple ``Count Sketch'' can be shown to be a subspace embedding if allowed to have enough rows.
(Count Sketch is sparser, but OSNAP has fewer rows.
There is some trade-off here that I'm not sure is actually completely theoretically understood.)

Anyway, the point is that we can just store some hash functions to compute $Sv$, and then learn $W'$ on that.
This is guaranteed to work just as well as having a very large $W$ and no $S$.

\subsection{Intuition from Locality Sensitive Hashing}
In locality sensitive hashing it is often necessary to build very large "codes".
That is, large sets of vectors that uniformely span the space.
For the best result, one needs to take in the order of $n^{\scet{n}}$ vectors, which is obviously completely ridiculous to imagine.
Hence, one creates multiple smaller sets of say $n^{\epsilon}$ vectors each, and then take the sum (or concatenation) of the sets (implicitly of course) as the total code.

This is all pretty obvious.
The interesting thing is that a product of smaller code is actually NOT a good approximation of a fully random (large) code.
In the sense that the geometric properties we need are not sufficiently similar to that of a fully random code.
What turns out to help is to take a random subset of the product code.

Intuition TLDR: Geometrically the product of multiple spheres isn't very much like a sphere. But if you sparsify the product, it DOES work.

Action TLDR: This is why we don't want to use the CE method of taking two tables with $\scet{n}$ vectors each as a replacement for a size $n$ table.
We need either more tables, or more rows in each table, so that there will be some ``unused combinations''.
By not using all combinations of the two (or more) tables, the code will be like the sparsified spherical product I described above.


